Multi-mode lasing in supercell plasmonic nanoparticle arrays

Multicolour light sources can be used in applications such as lighting and multiplexing signals. In photonic and plasmonic systems, one way to achieve multicolour light is via multi-mode lasing. To achieve this, plasmonic nanoparticle arrays are typically arranged in superlattices that lead to multiple dispersions of the single arrays coupled via the superlattice Bragg modes. Here, we show an alternative way to enable multi-mode lasing in plasmonic nanoparticle arrays. We design a supercell in a square lattice by leaving part of the lattice sites empty. This results in multiple dispersive branches caused by the supercell period and hence creates additional band edges that can support lasing. We experimentally demonstrate multi-mode lasing in such a supercell array. Furthermore, we identify the lasing modes by calculating the dispersion by combining the structure factor of the array design with an empty lattice approximation. We conclude that the lasing modes are the 74th $\Gamma$- and 106th $X$-point of the supercell. By tuning the square lattice period with respect to the gain emission we can control the modes that lase. Finally, we show that the lasing modes exhibit a combination of transverse electric and transverse magnetic mode characteristics in polarization resolved measurements.

==> latexmkrc <==
$sub_doc_output = 'output-subdoc';

@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {

             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}
